Extracting O*NET Features from the NLx Corpus to Build Public Use Aggregate Labor Market Data

Data from online job postings are difficult to access and are not built in a standard or transparent manner. Data included in the standard taxonomy and occupational information database (O*NET) are updated infrequently and based on small survey samples. We adopt O*NET as a framework for building natural language processing tools that extract structured information from job postings. We publish the Job Ad Analysis Toolkit (JAAT), a collection of open-source tools built for this purpose, and demonstrate its reliability and accuracy in out-of-sample and LLM-as-a-Judge testing. We extract more than 10 billion data points from more than 155 million online job ads provided by the National Labor Exchange (NLx) Research Hub, including O*NET tasks, occupation codes, tools, and technologies, as well as wages, skills, industry, and more features. We describe the construction of a dataset of occupation, state, and industry level features aggregated by monthly active jobs from 2015 - 2025. We illustrate the potential for research and future uses in education and workforce development.

==> scratch.tex <==

%Online job ad titles explain more than 90\% of the variance in wage and 80\% of education requirements \citep{marinescu_opening_2020}. We extract structured information on many parts of the job ad title that can explain variance in wage.

\section{titles}


%Toward a Public Use Aggregate Dataset of Online Job Ads by Deconstructing a Massive Corpus into Standardized Features
%\title{The Construction of Aggregate Labor Market Information from Online Job Ads}
%\title{Online job ads Data: Mapping O*NET Features to the NLx Corpus}
%\title{The Construction of a Public Dataset of Online Job Ads}
%\title{A Public Dataset of Online Job Ad Data}
%\title{A New Panel Job Ad Database from the NLx Corpus and Job Ad Machine Learning Models}
%Deconstructing the Massive NLx Job Ad Corpus Into Data to Build Public Use Labor Market Information 
%Job Ad Data: Mapping the NLx Corpus to O*NET Features
\section{intro}


% through \textcolor{red}{[NLx Research Hub? Academic Repository?]}

% and have sought to have it mapped to commonly used research taxonomies, such as

%Second, we make improvements to information collected by O*NET and job ad data by processing high volumes of real-time job ad data according to the standard taxonomies for understanding work developed by O*NET and adopted by researchers and supported by statistical research agencies. Third,

%We build these ML models with expert participation and curation.
\section{data}

%O*NET further links Generalized Work Activities (4.A.) to Abilities (1.A.) and Skills (2.A.).


%Studies adopting the task approach often treat jobs as bundles of tasks. 

%The task approach literature often adopts O*NET data to inform studies of change in the labor market.


%These scales rarely appreciate variation in tasks between jobs that are in the same occupation, or inter-firm or inter-industry variation in offshorability, teleworkability, or automatability.


%While much of the economics literature assumes that there is change in demand for tasks over time, 


%Papers that seek to measure occupational exposure to shocks using O*NET task data may draw faulty conclusions because the data is not designed to understand intra-occupational task heterogeneity or change over time.




%Aggregate labor market data today often involves a proliferation of proprietary skill and other taxonomies, rather than standard classification systems. 


%We evaluated and considered multiple providers of job ad data for this research. 




%, and provides the only independent assessment that seeks to compare job ad data from different sources. 
%In management, sociology, and economics research, aggregate job ad data are used to investigate employer concentration, questions in strategic management. Labor exchange data is

%Aggregate labor market data today often involves a proliferation of proprietary skill and other taxonomies, rather than standard classification systems. 

%Academic users are increasingly cautioned to understand both the fidelity of data generated in research using AI or machine learning models and the data provenance \cite{aea_ethics}.
%However, a major limitation for all research with job advertisements up to this point is the lack of researcher involvement in building scientific-use data from the unstructured text of job advertisements. We focus below on the sources of job ad data, and problems related to accessibility, replicability, and transparency. The central problem we seek to address is how little extant research develops tools for obtaining structured information from these text documents. 

%Carnevale \citet{carnevale2014understanding} first highlighted 


%A nascent research and practitioner ecosystem supported by NLx Research Hub has increased researcher engagement in 


%We transform the job description, zip code, and date fields from NLx that are present over 97\% of job ads  to create our dataset. We use NLx wage information where available for minimum (4.6\%) and maximum (4.15\%) wage ranges, and build a new comprehensive wage variable including wage information we extract from job ad text. We use company name from NLx for the 61\% of job ads where it is available, and transform company names into industry codes by a process described below. For wage and company name, we developed custom tools to extract these features, and then create a standardized wage variable and industry code to prepare the data for research use. For all other areas, we built entirely new data tools to extract O*NET features from job ad descriptions. 

%Table \ref{tab:nlx_feat} summarizes features in NLx and the percent of job ads with non-missing data for each feature. As can be seen in Column 2, NLx's structured metadata is incomplete.


%It therefore is difficult for researchers to use the data, and for that reason, much of the research using job ad data is based upon data purchased from a commercial provider.


% 

% \begin{table}[htbp!]
% \centering
% \csvreader[tabular=|l|c|,
%     table head=\hline \textit{Feature} & \textit{Percent of Job Ads}\\\hline,
%     late after line=\\\hline]%
%     {csvs/nlx_features.csv}{feature=\feature,jobpercent=\jobpercent}%
%     {\feature & \jobpercent}%
% \caption{Percent of Job Ads in NLx that include certain features}
%     \label{tab:nlx_feat}
% \end{table}


\section{JAAT}


%Tools we developed to extract O*NET features in Section \ref{sec:methods} include: TitleMatch (\ref{sec:titlematch}), TaskMatch (\ref{sec:taskmatch}), SkillMatch \ref{sec:skillmatch}, FirmNER \ref{sec:firm_extract}, and WageNER \ref{sec:wageextract}. 

% Section \ref{sec:titleocc} describes mapping from job title to occupation (O*NET 5.C and 5.E). Section \ref{sec:firm_name} describes extraction of firm names and mapping these firm names to an establishment-level business registry that allows us to provide industry-level aggregation. Section \ref{sec:geo} describes 

%Section \ref{sec:dwh} presents the design of the data warehouse and the resulting star schemas.

%We engage in inductive and deductive sampling of text, qualitatively analyze job ad language, and identify and label concepts we seek to code manually. For example, we developed novel dictionaries of benefits and shifts.


%, including description of validation efforts undertaken in the process of building training data. While there is no benchmark data for assessing the accuracy of NLP tools in this domain, in the Appendix, we compare our model's performance on non NLx data labeled by other means. 

%The occupation field in NLx is also restricted by licensing terms and conditions and cannot be used for research or many other purposes. 


% \begin{table}[htbp]
% \centering
% \resizebox{\linewidth}{!}{
% \begin{tabular}{l|ccccccccccccccccccccc|c}
% Validator & 0.80 & 0.81 & 0.82 & 0.83 & 0.84 & 0.85 & 0.86 & 0.87 & 0.88 & 0.89 & 0.90 & 0.91 & 0.92 & 0.93 & 0.94 & 0.95 & 0.96 & 0.97 & 0.98 & 0.99 & 1.00 & Agree \\ \hline
% \textsc{GPT-4o-mini} & 0.06 & 0.16 & 0.18 & 0.22 & 0.21 & 0.26 & 0.35 & 0.44 & 0.57 & 0.67 & 0.73 & 0.85 & 0.89 & 0.84 & 0.95 & 0.95 & 0.99 & 0.99 & 1.00 & 1.00 & 1.00 & \multirow{2}{*}{0.788} \\
% \textsc{Llama-3.3-70B} & 0.23 & 0.40 & 0.45 & 0.55 & 0.56 & 0.65 & 0.73 & 0.82 & 0.87 & 0.90 & 0.91 & 0.94 & 0.97 & 0.92 & 0.99 & 0.97 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 &  \\ \hline \hline
% Human 1 & x & x & x & x & x & x & x & x & x & x & x & x & x & x & x & x & x & x & x & x & x & \multirow{2}{*}{x} \\
% Human 2 & x & x & x & x & x & x & x & x & x & x & x & x & x & x & x & x & x & x & x & x & x & 
% \end{tabular}
% }
% \caption{Validation results for LLM-as-a-Judge and human coders on SkillMatch semantic matching. Results are given per similarity score (columns), and the values represent the percentage of correctly matched skills, as judged by the coders.}
% \label{tab:match_validation}
% \end{table}

%We initially found that 80\% of the job titles appearing in a random sample of job advertisements can be exact matched to at least one O*NET occupation code. A random audit revealed that 96.8\% of the positive identifications based on an exact match of an occupation were true positives. We bulk up the O*NET list of job titles with highly similar job titles from job ads. 

%To return occupation codes, TitleMatch embeds the O*NET sample of reported titles to allow the job title archetypes presented in O*NET to be scaled over job titles that are missing in the O*NET dictionary.  

%For the 20\% of non-matches, we used an embedding similarity model to match job titles to the closest similar entry in the O*NET dictionary. 


%We believe that simplifications such as this can be informative about the hierarchical distribution of postings in firms.


%We present several figures that illustrate model results and confirm that the TitleMatch tools, built with separate models and training data, provide converging results and are working as intended. We illustrate hierarchy values for all occupations, management occupations, and the chief executive occupation as well as personal care workers and supervisors of personal care workers. 


% \begin{itemize}
%     \item Total number of job ads: 137,964,605; rounded to 138M
%     \item Total number of tasks extracted: 585,003,714; rounded to 585M
%     \item Total number of job ads with at least one task extracted: 88,878,765; rounded to 89M. This is 64.5\% of all job ads.
%     \item The maximum number of different tasks extracted from a single job ad is 89.
% \end{itemize}

%For example, to study the risk AI poses to automation of jobs,  build novel measures and conduct an individual survey to identify a task's exposure to AI, and then use O*NET's data on the tasks within an occupation to extrapolate their findings to the labor market.




%We link the Data Axle unique code to unique codes for publicly traded firms such as CUSIP, GVKEY, and CIK, and indexes such as the S\&P 500, NASDAQ, etc. This enables future research that combines job ad data with publicly available information on firms. 
%and suggesting a very high degree of accuracy. 


% \begin{figure}
% \centering
% \caption{WageExtract: The percent of postings with wage information}
% \setlength{\tabcolsep}{5pt}% A
% \begin{tabular}{p{0.48\textwidth} p{0.48\textwidth}}
% \includegraphics*[width=0.45\textwidth]{pngs/has_wage2.png} &
% \includegraphics*[width=0.45\textwidth]{pngs/pay_transparency.png} \\
% \scriptsize{(a) From WageExtract and NLx Metadata} &
% \scriptsize{(b) Selected States with Pay Transparency laws, Florida, and Texas}  \\
% \label{fig:wage_extract}
% \end{tabular}
% \end{figure}


%NLx metadata is missing 38.7\% of firm names for the 2015-2025, similar to the 36\% missing in Burning Glass \citep{lancaster2019technology}.


%(described in Appendix \ref{sec:onet_data}) as well as custom dictionaries developed to supplement additional discovery and standard dictionaries (Appendix \ref{sec:std_dictionaries}). 

\section{Aggregation scratch}


%O*NET provides detail only at the occupational level and is infrequently updated. We address this barrier to understanding intra-occupational heterogeneity with real-time job ad data 


%Because we aggregate to industry and geography, our data will allow researchers to test hypotheses regarding variation in work patterns within and between regions and industries. For example, the observation within the U.S. (and globally) that employment systems have become more fragmented over recent decades, especially by industry \cite{katz_converging_2000}, could be tested with large-scale quantitative data. 


%available from \href{https://usa.ipums.org/usa/volii/1990LMAascii.txt}{IPUMS}. 

%and available at \href{https://www.huduser.gov/portal/datasets/usps_crosswalk.html}{https://www.huduser.gov/portal/datasets/usps\_crosswalk.html}).




%and the tools we developed to extract O*NET features in Section \ref{sec:methods}: TitleMatch (\ref{sec:titlematch}), TaskMatch (\ref{sec:taskmatch}), WageNER \ref{sec:wageextract}, FirmNER \ref{sec:firm_name}, and SkillMatch \ref{sec:skillmatch}.  


%Appendix \ref{sec:onet_data} provides a detailed description mapping of features we extract to the O*NET taxonomy. Appendix  




%\subsubsection{Low-Resource Computing}
%The suite of tools in JAAT can run in low-resource computing environments and extract data from hundreds of millions of job ads. Training and classification of these models was done on a single NVIDIA Quadro RTX 8000 GPU. Typical processing times for a single model run on the entire corpus are 10-14 days with this hardware.

%\subsection{SIC Code – PN/SM}



% \subsection{Data Warehouse}
% \label{sec:dwh}

% We structure and store the data in a data warehouse designed using dimensional modeling \cite{jukic2016database}.  There are two star schemas with shared dimensions.  We consider separately the set of tasks extracted from each job ad and the set of tools and technologies extracted from each job ad.  Thus, we have two fact tables.

% The Job\_Task fact table contains a tuple (row) for each task identified (extracted) from a particular job ad text.  The Job\_Tool fact table contains a tuple (row) for each tool or technology identified (extracted) from a particular job ad text.  The two fact tables share several dimensions. 

% The two star schemas, which form a galaxy, are shown in \ref{fig:star_schema}.

% \begin{figure}
%     \includegraphics[width=\textwidth]{pngs/Job_Task_Tool_Star_Schemav0_7.png}
%     \label{fig:star_schema}
% \end{figure}

% The Calendar dimension is a standard dimension derived from the date\_compiled field.  The lowest level of granularity of this dimension is month-year. Note that while date\_compiled is a full date, typical analysis of the data uses months, quarters and years, so the exact dates are not necessary. 

% \begin{comment}
% Describe that date\_compiled is assigned as the last date a job is seen and thus it makes sense not to put too much emphasis on the exact date but use the month instead as a better indicator.
% \end{comment}

% The Location dimension contains geographical information derived from the zipcode and include a hierarchy starting with fibs, commuter zone, city, and state. 


% \subsubsection{Methods and Model Development}

%(Neuendorf, 2017), 
%\cite{li_theoryon_2020}

%Describe it as a framework with ad hoc elements. We match models to the corpus and  

%Computational model - what is the right threshold so we are confident results are good? 

%how do you discover the categories? inherently manual? is there something generalizable? for tools and technologies. 

%For firm: 
% 1. general threshold - 0.8
% 2. short names - 0.9
% 3. common words - 0.9 

\section{firefighter e.g.}


%An illustration in Figure \ref{fig:shiny_tool} for the Firefighter occupation demonstrates how the information extracted from job ads aligns with -- and differs from existing O*NET data. 

% \begin{table}[htbp]
%   \centering
%   \begin{threeparttable}
    
%     \small 
    
%     % --- First Table (from Job Ads) ---
%     \justifying 
%     \textbf{A. Top Tasks from NLx Job Ad Data}
%     \par\medskip
%   %  \csvautobooktabular[respect all]{csvs/firefighter_tasks.csv}
%  \pgfplotstabletypeset[
%     col sep=comma, % Specify the separator
%     header=true,   % The CSV has a header row
%     string type,   % Treat all columns as text initially
%     columns/Importance/.style={column name=Importance, column type=l},
%     columns/Category/.style={column name=Category, column type=l},
%     columns/Task/.style={
%         column name=Task, 
%         column type={p{11cm}} % Wrap text in this column
%     },
%     every head row/.style={before row=\toprule, after row=\midrule},
%     every last row/.style={after row=\bottomrule},
%     ]{csvs/firefighter_tasks.csv}
%     \bigskip 
    
%     % --- Second Table (from O*NET) ---
%     \textbf{B. Top Tasks from O*NET Data}
%     \par\medskip
%   % Define the table structure manually for better control
%     \pgfplotstabletypeset[
%     col sep=comma, % Specify the separator
%     header=true,   % The CSV has a header row
%     string type,   % Treat all columns as text initially
%     columns/Importance/.style={column name=Importance, column type=l},
%     columns/Category/.style={column name=Category, column type=l},
%     columns/Task/.style={
%         column name=Task, 
%         column type={p{11cm}} % Wrap text in this column
%     },
%     every head row/.style={before row=\toprule, after row=\midrule},
%     every last row/.style={after row=\bottomrule},
%     ]{csvs/firefighter_tasks_onet.csv}
    
%     % --- Table Notes ---
%     \begin{tablenotes}[flushleft]
%       \small 
%       \item[] \textit{Note:} For the September 2015 - June 2025 period, 294,651 tasks are extracted from 26,987 job postings in the firefighter occupation. This table reports the top 15 based on data from an aggregated summary table on the top 10 tasks for each month and occupation.
%     \end{tablenotes}

%   \end{threeparttable}
%   \caption{The Top Fifteen Tasks for Firefighters in NLx Job Ad Data and O*NET Data.}
%       \label{tab:firefighter}
% \end{table}

% \begin{landscape}
% \begin{figure}[htbp]
%     \centering
%     \includegraphics[scale=0.25]{pngs/firefighters_diagnostics.png}
%     \\
%     \small
%     \justifying{\emph{Note:} An illustrative example of diagnostics information for the firefighter occupation using the Job Ad exploration tool. This illustrates the number of postings each month, the availability of wage and firm (industry) data for the occupation, and the average match scores for occupation and industry matching for this occupation. Data for from months with fewer than 200 observations are suppressed.}
%     \caption{A Job Ad Data Exploration Tool with Shiny}
%     \label{fig:shiny_tool}
% \end{figure}
% \end{landscape}


%By illustrating how select variables we construct have plausibility as indicators of job quality, we demonstrate that job ad data can be a useful contributor toward the development of novel measurements for ideas that have obtained theoretical relevance but lack empirical evidence or coherence upon an agreed measurement approach. Second, we demonstrate that this

\section{taskmatch results scratch}


% \begin{figure}[htbp!]
% \centering
% \caption{TaskMatch: The growth of project-based work}
% \setlength{\tabcolsep}{5pt}% A
% \begin{tabular}{p{0.48\textwidth} p{0.48\textwidth}}
% \includegraphics*[width=0.45\textwidth]{pngs/tasks_all.png} &
% \includegraphics*[width=0.45\textwidth]{pngs/tasks_software_developer.png} \\
% \scriptsize{(a) ç} &
% \scriptsize{(b) Top Tasks for Software Developer (15-1252.00).} \\
% \label{fig:tasks_projects}
% \end{tabular}
% \end{figure}




% \begin{figure}[htbp!]
% \centering
% \setlength{\tabcolsep}{5pt}% A
% \begin{tabular}{p{0.48\textwidth} p{0.48\textwidth}}
% \includegraphics*[width=0.45\textwidth]{pngs/fk_all.png} &
% \includegraphics*[width=0.45\textwidth]{pngs/fk_info.png} \\
% \scriptsize{(a) Fleisch Kincaid Readability Score for All Observations} &
% \scriptsize{(b) Fleisch Kincaid Readability Score for Information Sector.} \\
% \caption{Changes in the Readability of Job Ads}
% \label{fig:fk_read}
% \end{tabular}
% \end{figure}

%the growing appearance of several of the most frequently appearing technologies in computer and mathematical occupations, along with the growth in the appearance of AI related keywords, a list that includes terms from \cite{lou_ai_2021} as well as a novel list with more recent terms related to generative AI. 


%a similar decade-long climb in computer and mathematics occupations that involve the use of database, AI, and data analysis tool.


%Rapid changes of occupational tasks may be common in the aftermath of a technological shock, and job ads are a useful source of data to assess the impact of sudden changes in technology (CITE Horton and Tambe). 


%TaskMatch returns detailed descriptions of tasks within job advertisements, and can assist in spotting major trends changing the nature of work. We provide an overview of several seemingly important trends: first, .  

\section{practitioner use: occ report}


% \subsection{Applications for Practitioners: A Sample Occupational Report}

% We provide an abbreviated and illustrative report in Appendix \ref{sec:app_admin_report} for one occupation using the data exploration tool we develop to highlight how an O*NET informed by job ad data might improve the understanding of changes in labor markets for practitioners. Figure \ref{fig:occ_corr_time} illustrated a significant decline in the percent of all U.S. workers in the Office and Administrative Support occupations. To peer into possible changes within an occupation that is in decline as an overall share of the workforce, we examine Secretaries and Administrative Assistants, an intermediate level of aggregation (inclusive of 43-6011, 43-6012, 43-6013, and 43-6014). 

% An examination of a decade's worth of job ads demonstrates that in the Secretaries and Administrative Assistants occupations: 1) performing administrative activities as a percent of work activities and as a skill is in decline, 2) training others is a rising work activity, 3) working with and leading others and supervising people are rising skills in this occupation, 4) taking a proactive approach is also rising, and 5) at the task level, greeting, protecting property, and placing displays were the top 3 tasks in 2015, while in 2025, the top 3 were all related to assigning duties to others. 

% %These findings might be contrasted with O*NET data, which 

% %By way of comparison, O*NET data, based on a survey of an average of 123 workers workers at a single timepoint, is available on ONET online. A job-ad based analysis of this occupation, based on tens of thousands of job ads each month, is available for every occupation. 

\section{lane plug}
% especially with the community engaged in its archiving and construction and practitioner use \citep{Lane2024Democratizing,hirsch_2024}., 


\section{App Onet}


%to outsource or automate decisions that structure language phenomena into distinct and measurable concepts likely stunts research progress from developing useful knowledge \citep{abend_words_2023}. T


%Because O*NET structured data has been unable to be readily accessed through job ads, researchers using O*NET to examine the Computer and Information Research Scientists occupation rely on under 100 observations from 2018, and would not find data mining and ML in the list of the top 15 tasks.


%One limitation in this approach is that the task statements from O*NET may not be exhaustive in their coverage of emerging tasks written in job ads. We did not pursue the creation of novel task statements.


%However, when we inspect that top tasks in the legal occupations include several related to bartending, we judge these to be mistakes, and note them to be corrected in future rounds of building training data to differentiate the legal bar from the other sort.

\subsection{onet erd}
%Figure \ref{fig:onet_eer} illustrates the entity relationship diagram for the database, and early notes we made to prioritize certain tables. Toward the center left, in dark red, is the Content Reference Model, a table is the ``conceptual foundation of O*NET'' and that joins all major features of the O*NET database into a single unified taxonomy for  understanding the most important aspects of work. 



% \begin{figure}[!htbp]
%     \centering
%     \caption{O*NET 29.1 Entity Relationship Diagram}
%     \label{fig:onet_eer}
%     \includegraphics[width=.9\textwidth]{pngs/onet_eer.png}
%     \medskip
% \small 
% \\

% \justifying
% In green on the top left side of the figure are task statements and crosswalks to work activities. In the yellow box to the right are occupational values for task intensity calculated in O*NET. The crosswalks between work activities (4.A.) and skills (2.A.) and abilities (1.A.) are on the lower left side in dark yellow. The box in dark red to its right is the Content Reference Model that ties together the various tables of the database. In orange on the right are tables that we used or considered using. On the far right are tables in O*NET that were less relevant to this work.
% \end{figure} 


%https://github.com/phaiptt125/newspaper_project/blob/master/data_cleaning/assign_SOC.ipynb


%describes , and how tasks inform higher-level measures of work activities (O*NET 4.A, 4.D, and 4.E), which can be crosswalked to  and skills (2.A) within O*NET. 
\subsection{nav}
%Section \ref{sec:titlematch} describes the extraction of hierarchy (O*NET 4.B) and work context features (O*NET 4.C) from job titles.  Section \ref{sec:tools} describes generation of technologies (O*NET 5.F) and tools (O*NET 5.G). Section \ref{sec:wageextract} describes wage information extracted from job ads (O*NET 4.B.1.b.3). Section \ref{sec:jobtag} describes several additional features related to the organizational context (O*NET 4.B). Sections \ref{sec:fk} and \ref{sec:hhi} respectively describe construction of measures of readability (Fleish-Kincaid scores) (O*NET 3.B.1.A. Reading Comprehension - Entry Requirement)  and labor market concentration (HHI) (O*NET 6.A Labor Market Information). 


%We combine wage information from job ad text with structured salary information in NLx metadata, and achieve a minimum or maximum wage for \textcolor{red}{15\%} of job ads in total. We consolidate all wage information into minimum, maximum, and mid 'wage' variables that reflect the hourly rate of pay. We assume a 40 hour work-week for positions that report annual or monthly salary. 


%Celebrity Nonconformity	Hubbard et al. 2018



\section{Appendix methods}



% The harmonic mean of precision and recall (or F1-score) is frequently used to evaluate model performance. When using this metric, a high score (i.e., towards 1) is important to instill confidence that a trained model has not only learned the training data well, but can also reasonably generalize beyond it. We report F1 scores in Table \ref{tab:model_overview}, but do not rely solely on them.


% In cases where no taxonomy exists or existing taxonomies have insufficient detail, we follow in the tradition of interpretive text analysis \citep{gephart1997hazardous}: we engage in inductive and deductive sampling of text, qualitatively analyze real job ad language, label it manually, and use machines to scale unseen instances with embeddings. Validity in the content analysis tradition typically starts with keyword searches, and including strategic and random audits of labeled output to ensure high content validity \citep{neuendorf2017content}. Oversampling and manually annotating the most frequently occurring text patterns, random sampling from bins across the frequency distribution of match scores, and random sampling of text chunks labeled by models illustrates where problems occur and enhances the ultimate model performance.  

% For tasks and skills, to prevent false positives, we build two-stage models in which we first identify sentences as 'task' or 'skill' sentences with a binary ML classifier trained to recognize sentences containing task or skill descriptions relevant to the worker. We built initial lists of task and skill sentences with content from O*NET and ESCO, respectively. We then pass only the sentences that contain task or skill content on to a similarity search embedding model. 

% To augment dictionaries and rule-based approaches, we use word and sentence embeddings  \citep{li_theoryon_2020}. We thereby generalize from a dictionary to capture the occurrence of a concept. For embedding models, we typically begin with an existing dictionary, augment it with highly similar real job ad language, and embed the results to complete a search for similar text in the job ads. In some cases, we add supervised ML built with training data created from the dictionary and boosted by real job ad text identified by embeddings with a high match score following audits of the training data. 

\subsubsection{Appendix Validity}

%With any job ad data, there are issues likely to arise at multiple points along the path to accurate aggregate data, including in data collection procedures undertaken long before model accuracy enters the picture. 


%For each model, we validate that we achieve 90\% accuracy in the prediction above a match score threshold in a small random audit, and then add real job ad text strings to either training data for supervised ML or adopt the threshold for embeddings-based similarity search in the entire corpus. 


%With dictionaries, we build aggregate data at the level of the 'knowledge map' but possess the detail on the individual subcomponent features extracted. 

%We evaluate F-Scores to assess model performance against training data, and conduct repeated strategic and random audits of results and by revising and re-running models until satisfied.  Random audits assess global accuracy of results, but could miss high-frequency mistakes that distort the data (CITE). Strategic audits (CITE) either scrutinize the most frequently occurring results in order to eliminate the vast majority of false positives, or results at different levels of the match score distribution to assess model accuracy at different thresholds.

\subsection{Appendix TaskMatch}

% %Computational linguistic analysis methods did not succeed on the first attempt. 

% To identify which sentences in a job ad contain task information, we built a binary BERT-based classifier to identify task sentences – sentences that contains description of tasks a worker might perform on the job. To build this classifier, we used the 20,000 task statements from O’NET as a basis for training data. Next, we used an augmentation approach, where a random sample of 100,000 job ads was segmented into sentences, and using an Sentence Transformer embedding model \citep{reimers-gurevych-2019-sentence}, specifically \textsc{GTE-small} \citep{li2023generaltextembeddingsmultistage}, we matched the most and least semantically similar sentences, thus augmenting the dataset to contain other plausible task statements, as well as clear examples of “not-task” statements. 

% A manual examination of the augmented data suggested by embeddings confirmed that task statements were relevant, and the non-task sentences were irrelevant to task classification. In an additional step, a random audit of 1000 training data samples was performed to identify clear misclassifications resulting from the matching. This validation feedback was used to re-run the augmentation process. 

% In audits, we observed that while many of the false positives were false in a strict sense, the embedding model often captured interesting similarities between tasks and suggest general concepts that are false only in that they differ from the precise meaning of the O*NET task statements. In interactively testing the model on a small sample of individual job ads from different firms and sectors, while recall was at times an issue, the accuracy of results obtained was impressive. As we sought a highly precise model, we deployed TaskMatch with the 0.90 threshold.

% on 145 million job ads and extracted 430,744,609 task IDs in approximately two weeks running on a single NVIDIA Quadro RTX 8000 GPU.

\subsection{App Standard Dictionaries}
% \begin{table}[htbp]
% \centering 
% \small
% \caption{Standard Management Dictionaries - Variables and Citations}
% \label{tab:mgmt_dicts} 
% \csvautobooktabular[respect all]{csvs/mgmtcodebook1.csv}
% \end{table}

% \clearpage
% \begin{table}[htbp]
% \centering 
% \small
% \caption{Standard Management Dictionaries - Variables and Citations}
% \label{tab:mgmt_dicts2} 
% \csvautobooktabular[respect all]{csvs/mgmtcodebook2.csv}
% \end{table}


% \subsection{Standard Dictionaries from the Management Literature}
% \label{sec:std_dictionaries}

% Standard dictionaries from the management literature run on the job ads include the following: 

% \begin{itemize}
% \label{list:papers}
%     \item Recruiting signals \citep{banks_strategic_2018}:  Achievement Oriented Culture, Creative Culture, Development Early, Development, Inclusive Military,  Inclusiveness, Corporate Social Responsibility, Team Based Culture,  Values Based Culture, Well Being.
%     \item Long Term Orientation \citep{brigham_researching_2014}: Continuity, Futurity, Perseverance.
%     \item Time Horizon Words: Long term, Neutral, Short \citep{brochet_speaking_2015};  Long, Short \citep{desjardine_one_2019}.
%     \item  Training Feedback: Utility, Satisfaction  Glerum et al. In Press
%     \item Management Innovation \citep{heyden_conjoint_2015}: Change, Practices, Processes, Structures.
%     \item Digital Orientation \citep{kindermann_digital_2021}: All dimensions, Architecture configuration, Capabilities, Digital ecosystem coordination, Digital technology scope.
%     \item CreativitySpeak \citep{haselhuhn_investors_2022}.
%     \item TMT Attention \citep{levy_influence_2005}:  Board of Directors, Competitors, Computer Ind. Customer, Healthcare Ind. Semiconductor Ind. Dealers, Employees, Owners, Strategic Partners, Management. Foreign Operations and Markets, including: Africa, Asia Pacific, Europe, Latin America, Middle East, North America.
%     \item Ambidexterity \citep{mckenny_what_2018}: Exploitation, Exploration.
%     \item Entrepreneurial Orientation	\citep{mckenny_strategic_2018}: Autonomy, Aggressiveness, Inductive, Innovativeness, Proactiveness, Risk Taking, Competitor Orientation, Customer Orientation, Interfunctional Coordination, Long Term Focus, Profitability. \citep{short_construct_2009}: Autonomy, Aggressiveness, Inductive, Innovativeness, Proactiveness, Risk Taking
%     \item  Value Orientation \citep{moss_funding_2018}: Economic Value, Social Value, Environmental Value
%     \item Task Environment \citep{olsen_coordinated_2016}: Stakeholder. 
%     \item Corporate Social Responsibility (CSR) \citep{pencle_whats_2016}: Employee, Environment, Human Rights, Social and Community
%     \item Sustainability Orientation \citep{vaupel_role_2023}: Addition, Environmental, Social
%     \item Market Orientation  \citep{zachary_family_2011}: Customer Orientation, Competitor Orientation, Inter-functional Coordination, Long Term Focus, Profitability.
% \end{itemize}



% \clearpage
\section{Appendix Sample Occupational Report for Secretaries and Administrative Assistants.}
% \label{sec:app_admin_report}
% A Shiny App enables inspections of the data. This report illustrates some of the data available in a report focused on Secretaries and Administrative Assistants, and includes SOC codes 43-6011, 43-6012, 43-6013, and 43-6014. 

% \begin{figure}[!htbp]
%     \centering
%     \caption{Detailed Occupation Selected with Total Job Postings per Month Displayed}
%     \includegraphics[width=.9\textwidth]{pngs/434360_0_layout.png}
%     \label{fig:43460_skill}
%     \medskip
% \small 
% \\

% \justifying
% Based on an analysis of NLx Research Hub job ad data. Occupations matched with TitleMatch.  
% \end{figure} 

% \begin{table}[htbp] 
%     \centering % Centers the table on the page
%     \caption{Top 10 Tasks in 2025}
%     \label{tab:top10tasks}
%     \begin{tabular}{@{} r p{8cm} r @{}} % Defines column alignment:
%         % @{} removes extra space at the edges of the table
%         % r: right-aligned for rank
%         % p{8cm}: paragraph column of 8cm width for task description (allows text to wrap)
%         % r: right-aligned for value
%         \toprule
%         Rank & Task Description & Value \\
%         \midrule
%         1 & Assign duties to other staff and give instructions regarding work methods and routines. & 7746 \\
%         2 & Assign employees to specific duties. & 7537 \\
%         3 & Supervise and instruct assistants. & 4706 \\
%         4 & Refer guest problems or complaints to supervisors. & 4562 \\
%         5 & Assign duties to workers, and schedule shifts. & 4376 \\
%         6 & Maintain cleanliness of work area. & 3527 \\
%         7 & Teach library patrons basic computer skills, such as searching computerized databases. & 3470 \\
%         8 & Adhere to local, state, and federal laws, regulations, and statutes. & 3469 \\
%         9 & Oversee training programs. & 3247 \\
%         10 & Instruct patients, parents, teachers, or employers in communication strategies to maximize effective receptive communication. & 2964 \\
%         \bottomrule
%     \end{tabular}
% \end{table}

% \clearpage
% \begin{figure}
%     \centering
%     \caption{Change in Work Activity Composition over Time}
%     \includegraphics[width=.9\textwidth]{pngs/43460_work_activity.png}
%     \label{fig:43460_activities}
%     \medskip
% \small 
% \\

% \justifying
% Based on an analysis of tasks extracted with TaskMatch.  
% \end{figure} 


% \begin{figure}
%     \centering
%     \caption{Top Work Activities in 2025}
%     \includegraphics[width=.9\textwidth]{pngs/43460_top_activities_2025.png}
%     \label{fig:43460_top_activities_2025}
%     \medskip
% \small 
% \\

% \justifying
% Based on an analysis of tasks extracted with TaskMatch.  
% \end{figure} 

% \clearpage


% \begin{figure}
%     \centering
%     \caption{Top Work Activities in 2015}
%     \includegraphics[width=.9\textwidth]{pngs/43460_top_activities_2015.png}
%     \label{fig:43460_top_activities_2015}
%     \medskip
% \small 
% \\

% \justifying
% Based on an analysis of tasks extracted with TaskMatch.  
% \end{figure} 

% \begin{figure}
%     \centering
%     \caption{Top Skills in May 2025}
%     \includegraphics[width=.9\textwidth]{pngs/43460_top_skills.png}
%     \label{fig:43460_skills_top}
%     \medskip
% \small 
% \\

% \justifying
% Based on an analysis of skills extracted with SkillMatch.  
% \end{figure} 

% \begin{figure}
%     \centering
%     \caption{Change in Skill Composition Over time}
%     \includegraphics[width=.9\textwidth]{pngs/43460_skills.png}
%     \label{fig:43460_skills}
%     \medskip
% \small 
% \\

% \justifying
% Based on an analysis of skills extracted with SkillMatch.  
% \end{figure} 


\section{JOLTS cuts}
%Given that the average number of working days in a month (minus holidays and weekends) is 26 \citep{davis_establishment-level_2013}, 

% Based on the above analysis, we sought to assess the tightness of fit between different approaches to aggregating the NLx postings data and JOLTS data. We aggregate the national monthly count of NLx job postings from the monthly jobs file. For testing purposes, we create the monthly count of postings from a single monthly file (at time 0) and using the monthly file of one or more of the preceding or subsequent monthly files within a 4-month range. This `rolling sum' approach allows us to assess whether adding leading or lagging months to a focal month would improve the fit between our dataset and JOLTS data. 

% Figure \ref{fig:jolts_rolling_correlation} illustrates the correlation between alternative rolling aggregations of the monthly count and JOLTS monthly job openings data. The overall and yearly correlations illustrate several descriptive findings: 1) adding one  lagging month typically decreases the correlation, 2) the correlation has increased in recent years compared to earlier, and 3) there is a stronger correlation when adding 3 or 4 months of leading data following the publication of the monthly file. The overall correlation is 0.7 when adding three months of data, including for all years since 2020 (a year where both job postings and official statistics collections may have been especially affected by pandemic related challenges). Because gains after three months appear to be small, and based on the above analysis, researchers may choose to add leading data to each focal month's dataset for analysis purposes. 

% \begin{figure}[!ht]
%     \centering
%     \caption{The Correlation Between JOLTS and NLx Postings}
%     \includegraphics[width=\textwidth]{pngs/jolts_rolling_correlation.pdf}
%     \label{fig:jolts_rolling_correlation}
% \end{figure}


% drop job ads that have a date_compiled on the last day of the month, indicating that the job posting continues to be online in the next month, and 

\section{CRAML cuts}
% \subsection{JobTag (CRAML)}

% A list of rules and dictionary items, given a priority level, and a corresponding tag, are ‘extrapolated’ or ‘bootstrapped’ over a text collection. Rules in this framework refer to semantic rules, or chunks of texts validated to be representative of a concept or class. Extrapolation of rules to text assists in rule validation, as extrapolation converts the set of rules into an extended dataset, matching all rules to instances of the rule found in a sample of the text, tagging each text chunk according to the user’s encoding of each rule. Priority level of rules determines the order in which a rule is considered: lower priority rules can be over-written by a subsequent rule with a higher priority. 


% When a rule set is “extrapolated” to a corpus it yields a structured dataset of accurately classified texts – a training dataset of user-defined labels mapped to texts, which serve as necessary input to ML training procedures. Context Rule Assisted Machine Learning (CRAML) is open-source software we developed to bridge user-defined rule sets and advanced NLP methods. As a method, CRAML yields quality, labeled datasets that can be used to train a ML classifier, while integrating qualitative and interpretive research techniques that give researchers the power to steer analysis and control measurement of a phenomena within a text. 

% CRAML trains a binary classifier for each tag, currently preferring the usage of random forest classification models. It returns “tabular data – variables in columns, cases in rows” \citep{lazer2017data}. Because the ML model returns only a 0 or a 1, data outputs are interpretable as indicating the presence or absence of the concept tag in the document.

% CRAML is computationally efficient. Users pre-select keywords and context windows to reduce inputs to only the plausibly relevant text in a document collection in both training and classification. An added performance benefit when removing irrelevant or non-essential information is to reduce noise and build a highly focused ML classification model that is run on windows of text within the document, rather than the whole document. Finally, the use of lightweight, “shallow” ML models (currently, random forest classifiers) allows CRAML-trained models to be run efficiently even on lower-resource systems. A limitation is that researchers must manually add each item to create dictionaries and rule sets, as well as the use of shallow models which sometimes may struggle with capturing semantic nuances such as negation.



%is \textcolor{red}{forthcoming with publication? available at a URL?}.

\section{tools and techs}
%We also leverage the available list of tools and technologies from O*NET to demonstrate the changes in several of the most frequently appearing technologies in computer and mathematical occupations, along with the growth in the appearance of AI related keywords, a list that includes terms from \cite{lou_ai_2021} as well as a novel list with more recent terms related to generative AI. Figure \ref{fig:ai_techs} illustrates that as a percent of all job postings in the computer and mathematical occupations, products related to databases appear most frequently, with AI terms rising rapidly in the mathematical sciences and exceeding the percent of data analysis software in several months. 

\section{Job Quality Indicators}



%Predicting Wage from Title Features}



% \begin{figure}
%     \title{Boxplot NYC Job Ad Career Levels and TitleMatch Hierarchy Prediction}
%     \includegraphics[width=\textwidth]{kdens_title_hierarchy_simp.png}
%     \label{fig:titles_kdens}
% \end{figure}

%and 17 additional detailed codes for levels that are reduced here to 6 ascending levels of responsibility.




%We then deployed strategic audits of 500 titles matched within bins of the similarity score. 



%In version 1, we found that the precision of the model falls below 0.60 below cosine similarity scores of 0.92 , and performs well above 0.92. With 83\% of observations matched at a similarity score of 0.92 or above, based on analysis of the distribution of match scores and audited data, a conservative if admittedly ballpark estimate of overall model accuracy on the full NLx corpus is 74 percent. 

%TitleMatch’s use of embeddings bridges the incompleteness of dictionaries. 


